Span-ConveRT: Few-shot Span Extraction for Dialog with Pretrained Conversational Representations

We introduce Span-ConveRT, a light-weight model for dialog slot-filling which frames the task as a turn-based span extraction task. This formulation allows for a simple integration of conversational knowledge coded in large pretrained conversational models such as ConveRT (Henderson et al., 2019). We show that leveraging such knowledge in Span-ConveRT is especially useful for few-shot learning scenarios: we report consistent gains over 1) a span extractor that trains representations from scratch in the target domain, and 2) a BERT-based span extractor. In order to inspire more work on span extraction for the slot-filling task, we also release RESTAURANTS-8K, a new challenging data set of 8,198 utterances, compiled from actual conversations in the restaurant booking domain.

==> 05-rw.tex <==
If there's space (highly unlikely) - write one quarter of a page about: 1) pretraining for conversational applications and its potential; 2) summarise previous work on span/value extraction for dialog.
